RNNPool: Efficient Non-linear Pooling for RAM Constrained Inference

Standard Convolutional Neural Networks (CNNs) designed for computer vision tasks tend to have large intermediate activation maps. These require large working memory and are thus unsuitable for deployment on resource-constrained devices typically used for inference on the edge. Aggressively downsampling the images via pooling or strided convolutions can address the problem but leads to a significant decrease in accuracy due to gross aggregation of the feature map by standard pooling operators. In this paper, we introduce RNNPool, a novel pooling operator based on Recurrent Neural Networks (RNNs), that efficiently aggregates features over large patches of an image and rapidly downsamples activation maps. Empirical evaluation indicates that an RNNPool layer can effectively replace multiple blocks in a variety of architectures such as MobileNets, DenseNet when applied to standard vision tasks like image classification and face detection. That is, RNNPool can significantly decrease computational complexity and peak memory usage for inference while retaining comparable accuracy. We use RNNPool with the standard S3FD architecture to construct a face detection method that achieves state-of-the-art MAP for tiny ARM Cortex-M4 class microcontrollers with under 256 KB of RAM. Code is released at https://github.com/Microsoft/EdgeML.

==> TabsNFigs/renet.tex <==
\begin{wrapfigure}{r}{0.5\columnwidth}
\vspace{-3mm}
	\centering
	\includegraphics[width=0.5\columnwidth]{TabsNFigs/images/renet.pdf}
	\caption{ReNet block when used as a replacement layer similar to RNNPool}
\label{fig:renet}	
\vspace{-3mm}
\end{wrapfigure}

==> TabsNFigs/rpool-face-m4.tex <==
\begin{table}[h]
\centering
    \caption{\small The architecture of \rpool-Face-M4}
\begin{tabular}{ c | c | c | c | c | c }
      \toprule
	  {Input} & {Operator} & $t$ & $c$ & $n$ & $s$\\
	  \midrule
	  $320 \times 240 \times 1$ & conv2d $3\times3$ & 1 & 4 & 1 & 2\\
	  $160 \times 120 \times 4$ & \rpoollayer & 1 & 64 & 1 & 4\\
	  $40 \times 30 \times 64$ & bottleneck & 2 & 32 & 1 & 1\\
	  $40 \times 30 \times 32$ & bottleneck & 2 & 32 & 1 & 1\\
	  $40 \times 30 \times 32$ & bottleneck & 2 & 64 & 1 & 2\\
	  $20 \times 15 \times 64$ & bottleneck & 2 & 64 & 1 & 1\\
	  \bottomrule
  \end{tabular}
 \label{tab:rpool-m4}
 \end{table}

==> TabsNFigs/rpoolillustration_bak.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{TabsNFigs/images/prnn_module.pdf}%
    \qquad
    \includegraphics[width=0.4\columnwidth]{TabsNFigs/images/prnn_patching.pdf}%
    \caption{\textbf{(left)} An \rpool operator. \textbf{(right)} An \rpoollayer composed with strided \rpool operators with shared weights.}%
    \label{fig:PRNN}%
\end{figure}

==> TabsNFigs/vww_imagenet_side_by_side.tex <==
\begin{figure*}[t!]
  \centering
  \begin{minipage}[t]{0.48\columnwidth}
    \includegraphics[width=\columnwidth]{TabsNFigs/images/vww.pdf}
    \vspace{-18pt}
    \caption{\small Visual Wake Word: MobileNetV2-\rpool requires
             $8\times$ less RAM and 40\% less compute than
             baselines. We cap our number of parameters to $\leq
             250$K instead of $290$K allowed by MobileNetV2
             (0.35$\times$). ProxylessNAS used $242$K parameters.}
    \label{fig:vww}
  \end{minipage}
  ~
  \begin{minipage}[t]{0.50\columnwidth}
  \centering
  \scriptsize
    \vspace{-78pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l c c c c}
      \toprule
      \multicolumn{1}{l}{Method} & {Peak RAM} & {Params} & {FLOPs} & {Accuracy} \\
      \midrule
      MobileNetV1 & 3.06MB & 4.2M & 569M & \textbf{69.52\%}\\
      MobileNetV1-ReNet & 0.77MB & 4.2M & 487M & 66.90\%\\
      MobileNetV1-\alg & \textbf{0.77MB} & \textbf{4.1M} & \textbf{417M} & 69.39\% \\
      \midrule
      MobileNetV2 & 2.29MB & 3.4M & 300M & \textbf{71.81\%} \\
      MobileNetV2-ReNet & 0.24MB & 3.6M & 296M & 66.72\% \\
      MobileNetV2-\alg & \textbf{0.24MB} & \textbf{3.2M} & \textbf{226M} & 70.14\% \\
      %   \midrule
      %   EfficientNet-B0 & 2.29 MB & 5.3M & 390M & \textbf{76.30}\\
      %   EfficientNet-B0-\alg & \textbf{0.25 MB} & \textbf{5.2M} & \textbf{330M} & 72.47\\
      \bottomrule
    \end{tabular}}
\caption{\small Comparison of resources and accuracy with
    MobileNets for ImageNet-1K.}
    \label{tab:imagenet}
  \end{minipage}
  \vspace{-17pt}
\end{figure*}
